Vortex: OpenCL Compatible RISC-V GPGPU

The current challenges in technology scaling are pushing the semiconductor industry towards hardware specialization, creating a proliferation of heterogeneous systems-on-chip, delivering orders of magnitude performance and power benefits compared to traditional general-purpose architectures. This transition is getting a significant boost with the advent of RISC-V with its unique modular and extensible ISA, allowing a wide range of low-cost processor designs for various target applications. In addition, OpenCL is currently the most widely adopted programming framework for heterogeneous platforms available on mainstream CPUs, GPUs, as well as FPGAs and custom DSP. In this work, we present Vortex, a RISC-V General-Purpose GPU that supports OpenCL. Vortex implements a SIMT architecture with a minimal ISA extension to RISC-V that enables the execution of OpenCL programs. We also extended OpenCL runtime framework to use the new ISA. We evaluate this design using 15nm technology. We also show the performance and energy numbers of running them with a subset of benchmarks from the Rodinia Benchmark suite.

==> __back.tex <==
\section{Background}
\label{sec:back}

\subsection{Background of POCL}
\label{subsec:pocl}
 
POCL is an open-source Performance Portable OpenCL Implementation which supports various types of target devices including general purpose processors (e.g. x86, ARM, Mips), General Purpose GPU (e.g. Nvidia), and custom TCE-based accelerators \cite{TCE}. The custom accelerator support provides an efficient solution for enabling OpenCL applications to use hardware devices with specialized acceleration (e.g. SPMV, GEMM). Figure \ref{fig:pocl} illustrates the system architecture of the POCL framework, which includes a runtime shared library implementing the OpenCL API and an LLVM-based back-end compiler for compiling the kernels. 

The POCL runtime implements a the device-independent common interface where each device target implementation plug into to specialize particular operations. This device independent layer implements the common operations needed by the devices such as the compiler driver, the file system abstraction, the memory abstraction, the synchronization and thread library. Figure \ref{fig:pocl_cc} illustrate the sequence diagram of the compilation flow across the various runtime layers, from when the kernel is created to the actual execution on the target device. Among the destination targets, POCL can also export PTX for NVidia devices and HSAIL \cite{HSAIL} IR for HSA compatible devices. At runtime, POCL invoke the back-end compiler with the provided OpenCL kernel source or SPIRV \cite{SPIRV} IR. 

The POCL back-end compiler process the provided kernel and apply a custom set of workgroup transformation passes on the kernel to handle barriers and implement low-level device-specific parallelization. There is also a built-in library that implements optimized device-specific OpenCL functions such as math operations (e.g. sin(), cos(), tan()). The reason for supporting this custom library is to provide more efficient implementations of those routine than what LLVM would produce by default. It also enables direct access to custom device instructions when targeting TCE-based accelerators. POCL supports target-specific execution models including SIMT, MIMD, SIMD, and VLIW. On platforms supporting MIMD and SIMD execution models such as CPUs, the POCL compiler attempts to pack as many OpenCL work-items in the work-goup to the same vector instruction if SIMD is supported, then the POCL runtime will distribute the remaining work-items among the active hardware threads on the device with provided synchronization using the Pthread library. On platforms supporting SIMT execution model such as GPUs, the POCL compiler delegates the distribution of the work-items to the hardware to spread the execution among its various SIMT cores, relying on the device to also handle the necessary synchronization. On platforms supporting VLIW execution models such as TCE-based accelerators, the POCL compiler attempts to "unroll" the parallel regions in the kernel code such that the operations of several independent work-items can be statically scheduled to the multiple function units of the target device.

\begin{figure}
  \centering
  \includegraphics[width=4in]{figs/pocl_system_architecture}
  \caption{POCL Systems Architecture}
  \label{fig:pocl}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=5in]{figs/pocl_compilation_flow}
  \caption{POCL Compilation flow}
  \label{fig:pocl_cc}
\end{figure}1


==> __evaluation.tex <==
\section{Evaluation}
\subsection{Evaluation Methodology}
\subsubsection{Simulator for exploring ISA options}

We propose five different ISAs for our initial version of Vortex Designs. We will explore other ISA design options using a functional simulator, simX. 

simX is a C++ cycle accurate simulator for Vortex RISC-V GPGPU.Figure~\ref{fig:simX} shows the overall view of the simulator. Its impact on the research process is significant as it enables the following: 1) Very quick ISA extensions and performance evaluations, 2) Software targeted research like compiler and algorithms techniques, and 3) dramatically improves and speeds up the hardware development process.

Because simX is built on top of a C++ instruction level emulator that produces trace objects, which are then fed into simX’s pipeline, the actual instruction execution happens in the emulator. Thus, for new ISA extensions to be implemented, the majority of the modifications will be done in this single functioned emulator, leaving the focus on the flow of the outputted trace objects through the simulated pipeline. This allows for very easy evaluations of multiple control flows and ISA research. Moreover, because simX is written in C++, executing benchmarks could be orders of magnitude faster than simulating the RTL. 

simX is also very beneficial for compiler and algorithms research. Adding performance counters and analyzing the microarchitectural is much more feasible and quicker to implement in simX. This analysis of microarchitectural events builds a bridge between high-level code and hardware events. This is possible by analyzing the values of the performance counters and the frequency of microarchitectural events for different programs.

Once the ISA has been finalized, and the performance and the benefits have been evaluated, simX also improves the hardware development process in case the hardware cost also needs to be evaluated. It’s a very important tool for debugging, as the whole microarchitectural state could be dumped for every cycle, which would be compared to the microarchitectural of the RTL for verification. In addition, since the ISA would have already been implemented in simX, it gives a much more clear path on the exact modifications that need to be changed to support the ISA on the RTL.   

\begin{figure}
    \centering
    \includegraphics[width=4in]{figs/simx.pdf}
    \caption{An overview of the simulator diagram}
    \label{fig:simX}
\end{figure}

\subsection{Benchmarks}
In this project, first, we will target to pass run the openCL testing benchmark, which gives the basic testing features. 
(https://openbenchmarking.org/suite/pts/opencl). The target application benchmark suites are Rodinia (https://rodinia.cs.virginia.edu/doku.php), Shoc (https://github.com/vetter/shoc/wiki), NPB (http://aces.snu.ac.kr/software/snu-npb/)  and GraphBig (https://github.com/graphbig/graphBIG).
GraphBig is developed by PI-Kim's research group using CUDA. In this project, we will convert the CUDA based GraphBig benchmark into OpenCL benchmark. GraphBig includes various graph algorithms (BFS, SSSP, Connected components etc.) which are crucuial to evaluate many graph algorithms. 


\subsection{Microarchitecture Design space explorations}

Area and power overhead for different warp/SIMD width results 

\subsection{Placement and layout} 
Layout and placement of the chip. 


==> __intro.tex <==
\subsection{Introduction}
\label{sec:introduction}
The current challenges in technology scaling \cite{Dark-Silicon} are pushing semiconductor industry towards hardware specialization, creating a proliferation of heterogeneous systems-on-chip, delivering orders of magnitude performance and power benefits compared to traditional general-purpose architectures. This transition is getting a significant boost with the advent of RiscV \cite{RiscV} with its unique modular and extensible ISA, allowing a wide range of low-cost processor design for various target applications. As these processors become specialized, often extending the existing ISA with domain-specific instructions, a challenge arises on how to program them and take advantage of their new capabilities. OpenCL \cite{OpenCL11} is currently the most widely adopted programming framework for heterogeneous platforms available on mainstream CPUs, GPUs, as well as FPGAs \cite{AOCL} and custom DSPs \cite{TIDSP}. Adopting OpenCL across all devices in heterogeneous platforms greatly simplifies the design and implementation of the software stack that drives these platforms, allowing OpenCL applications to scale efficiently as new computing devices are introduced. Additionally, there is a large ecosystem of existing parallel applications written in OpenCL that will now be able to run on those devices.

There is currently no publicly available implementation of OpenCL for RiscV accessible to the open-source community. This is mainly because the vector ISA extension \cite{RiscVV} for RiscV is still under development. However, there are existing implementations of RiscV processors with multi-core support \cite{AX25MP}, including some with custom ISA for parallel processing \cite{ara} \cite{MANIC}, including ours \cite{Vortex} that could greatly benefit from OpenCL to increase adoption. Implementing a flexible compiler framework that makes it easy to port OpenCL to RiscV-based heterogeneous parallel processors is a challenge and this project aims at solving this programming gap.   

There exists a wide range of open-source implementations of OpenCL targeting various architectures including X86 with Beignet \cite{Beignet}, Intel Neo \cite{IntelNeo}, Nvidia with libclc \cite{libclc}, AMD with Clover \cite{Clover}, ROCm \cite{ROCm}, ARM with POCL \cite{POCL}, TI DSPs with Shamrock \cite{Shamrock}. POCL \cite{POCL} implements a flexible compilation backend based on LLVM, allowing it to support a wider range of device targets including X86, ARM, AMD, Nvidia, and TCE \cite{TCE}, making it our preferred choice for implementing a RiscV backend. The technical knowledge of our working group in this space with prior work on GPGPU design and implementation \cite{Harp,Vortex}, compiler optimization~\cite{ref1-1,ref1-2,ref1-3,ref1-4} and experience with LLVM \cite{LLVM,ref2-1,ref2-2,ref2-3} compiler toolchain will provide us the intellectual resources for completing this project. 


% LocalWords:  sec:introduction paralleizable subsubsection ai-rp Tensorflow
% LocalWords:  resnet16 ryoo17privacy includegraphics linewidth mliot hline vgg
% LocalWords:  fig:overview table:task simonyan2014two ssd subsec:target


==> __outline.tex <==


\section{introduction}
why GPGPU with RISC-V ? 
Why supporting OpenCL? 

What's the contributions ?

Showing that only five instructions are need to support GPGPU 


\section{background}

\subsection{OpenCL programming models} 
probably not much 

What ISA needs support for GPGPU? 

\subsection{OpenCL requirements} 
Background of POCL 



\section{ISA extensions} 

\subsection{ISA requirements for programming primitives}
Design space explorations 

how did we get these five instructions? 

Any other alternative design options ? 


\section{Micro-architecture of Vortex}

\section{POCL extensions}


\section{Evaluation}

(1) can it really run all OpenCL benchmarks? 
OpenCL benchmarks 

(2) RISC-V vector vs. Vortex 

(3) Hardware synthesize results 

\section{related work}

\section{conclusions}



==> __related.tex <==
\section{Related Work}
\label{sec:related}
  


Table~\ref{tab:opencl} summarizes the current status of open-source OpenCL run-time  implementations. POCL shows the most promising path since it supports the most number of ISA, particularly the support for ARM. We decided to use the POCL framework as a baseline for implementing an OpenCL support for RISC-V. 
  
\begin{table}[!h]
\centering
\begin{tabular}{|c||c|c|c|c|}
\hline
Name & Version & Target & status & Url \\ \hline 
Intel Bignet & 2.0 & x86 & Closed & https://cgit.freedesktop.org/beignet
\\ \hline
Intel Neo & 
2.1 & 
X86 & 
Active & 
https://01.org/compute-runtime  \\ \hline
POCL & 
1.2 & 
x86, ARM & 
Stable & 
https://github.com/pocl/pocl  \\
 & 
 & 
AMD, TCE, PTX & 
 & 
 \\ \hline

ROCm  & 
1.2 & 
AMD & 
Stable & 
https://github.com/RadeonOpenCompute  \\ \hline 
TI-OpenCL  & 
1.1 & 
TI & 
Closed & 
https://git.ti.com/opencl/ti-opencl  \\ \hline 
Shamrock & 
1.2  &
TI & 
Active & 
https://git.linaro.org/gpgpu/shamrock.git 
\\ \hline 
libclc & 
1.2 & 
AMD, PTX & 
Closed & 
https://libclc.llvm.org/  
\\\hline 
Clover & 
1.1 & 
AMD & 
Closed & 
https://people.freedesktop.org/~steckdenis/clover/  
\\ \hline 
\end{tabular}
\caption{Open Source Open CL implementation status}
\label{tab:opencl}
\end{table}
 


==> __vector.tex <==
\section{Discussions with Vector ISAs}

Another approach to extend RISC-V to support parallel 

programming is using vector instructions. 

Code examples for simple kernels 

We need a figure like this for RISC-V vector and Vortex. 

code examples for graph traversals 

BFS example for vector coding and GPGPU coding. 

\begin{figure*}
    \centering
    \includegraphics[width=6in]{figs/vector_code.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}












==> __vortex.tex <==
\subsubsection{ISA extensions}

\label{sec:RISC-V ISA Extenstion}

This section describes our proposed ISA extension that enables building SIMT using RISC-V. To accomplish the desired behaviour, we introduce five new instructions, and a thread mask register, to the RISC-V ISA, which were inspired by HAPR ISA~\cite{Kersey:2017:LSC:3132402.3132426}. The proposed five new instructions are RISC-V R-Type instructions and fit in one opcode. These instructions are intended to be the minimal set of instructions to introduce SIMT functionality to an architecture that supports OpenCL. They are designed to address the three new concepts that SIMT introduces: hardware warps, hardware threads, and control divergence.


\paragraph{Warp Control} \label{wc}

The \textit{wspawn} instruction is intended to address the introduction of hardware warps to the architecture; The instruction spawns w number of inactive warps at a specific PC values. There are two major differences between this instruction and the old Vortex ISA/Harp ISA: 1) It spawns an arbitrary number of warps in one instruction, compared to the old ISA where 32 instructions had to be executed to spawn 32 warps, and 2) It does not require copying register values from one register file to another, thus it's more efficient.

\begin{center}
\begin{tabular}{ |c| } 
 \hline
wspawn \%warps, \%PC \\
 \hline
\end{tabular}
\end{center}

\paragraph{Thread Control} \label{tc}

We propose \textit{tmc} instruction to address the introduction of SIMD lanes. \textit{tmc} instruction activates and deactivates lanes by controlling the thread mask register for the executing warp. The thread mask register could be read as a Control and Status register (CSR) and contains a bit for each thread singnifying whether the thread is currently active or not. For example, if \%NumThreads is equal to five, then lanes zero to four will be activated and the five least significant bits of the thread mask will be set to one. \textit{tmc} instruction is also used to halt execution of warps by setting \%ThreadNum equal to zero.

\begin{center}
\begin{tabular}{ |c| } 
 \hline
tmc   \%NumThreads \\
 \hline
\end{tabular}
\end{center}

\paragraph{Control Divergence}

\textit{split} and \textit{join} instructions are used to handle control divergence. Control divergence, which occurs when the threads in the same hardware warp want to follow  distinct execution paths, is handled by a hardware immediate postdominator (IPDOM) stack~\cite{Kersey:2017:LSC:3132402.3132426}. The \%predicate is set by any of the 32 general-purpose registers and it is considered true by the \textit{split} instruction if there's a non-zero value stored in the register. \textit{split} instruction pushes information about the current state of the thread mask and the predication result for all hardware threads into the IPDOM stack and \textit{join} pops out of the IPDOM stack (more details in Section~\ref{Control Divergence}). If a \textit{join} is executed without a corresponding \textit{split}, an exception will be thrown.

\begin{center}
\begin{tabular}{ |c| } 
 \hline
split \%predicate \\
join                \\
 \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ |c| } 
 \hline
split \%numWarps, \%barrierID  \\
 \hline
\end{tabular}
\end{center}

\paragraph{Barriers}
\textit{bar} instruction is used as a hardware barrier for warps. When a warp executes the \textit{bar} instruction its execution is halted until numWarps execute the \textit{bar} instruction with the same barrierID. In addition, the value of the barrierID encodes whether this barrier is private to the core or is public to other cores.These private and public will be used to control work-group level synchronizations. Understanding different types of barrier ISA options and exploring design choices is one of the major tasks of our ISA extension studies. Barrier instructions are also strongly connected with memory models and program models, which we will also explore together. 

\subsubsection{Microarchitecture}
\label{sec:Microarchitecture Implementation}



\ignore{
\begin{table}[h!]
\centering
\caption{Our proposed SIMT ISA extension.}
\begin{tabular}{||c | c||} 
 \hline
 Instructions & Description \\ [0.5ex] 
 \hline\hline
 wspawn & Spawn new warps.  \\ 
 tmc & Change the thread mask to activate threads\\
 split & Control flow divergence \\
 join & Control flow reconvergence \\ [1ex]
 bar & Hardware warp barrier
 \hline
 \hline
\end{tabular}
\label{table:isa}
\end{table}
}

\begin{figure}
    \centering
    \includegraphics[width=4in]{figs/vortex_microarchitecture.pdf}
    \caption{Vortex Micro architecture}
    \label{fig:vortex_micro}
\end{figure}

The aim of Vortex GPGPU is to make a lightweight GPGPU that is highly customizable to target specific applications. Vortex GPGPU is a 32-bit 5-stage pipeline that supports RISC-V's integer and multiplication extensions (RV32IM) on top of the instructions mentioned in Section ~\ref{sec:RISC-V ISA Extenstion}. Compared to a basic RISC-V pipeline, Vortex has 1) a hardware warp scheduler that contains the PC and thread mask registers and an IPDOM stack for each hardware warp 2) A banked GPR that contains the general registers for each thread in each warp, 3) A banked Dcache module that supports multiple memory accesses per cycle, and 4) a shared memory module. In addition, the execute stage has a vector ALU that supports the SIMD lanes; However, the number size of the Vector ALU does not have to be equal to the number of hardware threads or lanes available. Thus, the latency of the execute stage will depend on the number of execution units in the configuration. Vortex supports a fully customizable warp and threads per warp configuration, L1 cache, and a banked shared memory module. An instruction being executed by a warp is only fetched and decoded once, but executes on the operands and destination registers for each hardware thread in a warp.

\paragraph{Warps} \label{Warp Scheduler}

The Issue stage contains a warp scheduler which implemented as a fine-grain scheduler which is a lightweight scheduler that and hides the latency for hazards for each warp. It stores a state that keeps track of which hardware warps are active and it supports the proposed Vortex ISA. In addition, issue stage also contains the thread mask and IPDOM stack, which handles control divergence. Thus, all the ISA modifications is implemented there as the hardware modifications required to support the ISA are very little.

\paragraph{Control Divergence} \label{Control Divergence}

One of the biggest challenges in SIMT processors is control divergence which leaves the pipeline highly underutilized because of its dynamic nature~\cite{Fung:2007:DWF:1331699.1331735}. However, to maintain a simplistic approach, a hardware IPDOM stack~\cite{Kersey:2017:LSC:3132402.3132426} is used to handle control divergence. The IPDOM stack works by maintaining a private thread mask register for each warp that stores a mask of the current running threads. When a \textit{split} instruction is reached, the current state of the thread mask and the inverse of the new thread mask, along with PC+4, are pushed onto the IPDOM stack. The next instruction continues with the new thread mask. When \textit{join} instruction is reached, the stack is popped and the pipeline either jumps to the PC popped from the stack, or falls through to the current PC+4.


\paragraph{Memory}

Similar to Volta architecture, Vortex supports both an L1 data cache and shared memory module~\cite{Jia2018DissectingTN}. The L1 cache implementation is parameterizable by number of banks, number of ways, cache size, and block size. Because the data cache is banked, Vortex could achieve high memory throughput given there are no bank misses.

Moreover, the shared memory module is extremely parallelizable. Each hardware thread has a one-cycle access if there are no bank misses. Vortex matrix library is optimized to reduce bank conflicts. The shared memory module is mapped to addresses 0xFF000000 to (0xFF000000 + shared memory size). This address space is interleaved for each bank by word; The word at 0xFF000000 is stored in bank 0, 0xFF000004 is stored at bank 1, ... for a number of banks equal to the number of hardware threads in the configuration.



==> discussion.tex <==
\section{RISCV Vector Extension Discussion}
\label{sec:related}

\begin{outline}
\1 What are the building blocks to enable a vector processor?
\1 ISA's comparison
\1 Architecture general building blocks
\1 micro-benchmark execution analysis
\1 Another approach to extend RISC-V to support parallel 
\1 programming is using vector instructions. 
\1 Code examples for simple kernels 
\1 We need a figure like this for RISC-V vector and Vortex. 
\1 code examples for graph traversals 
\1 BFS example for vector coding and GPGPU coding.
\end{outline}

% \pagebreak
% .
% \pagebreak
